Less Is More: Fast and Accurate Reasoning with Cross-Head Unified Sparse Attention

Large reasoning models achieve strong performance through test-time scaling, but this incurs substantial computational overhead due to long decoding from short prompts. While sparse attention can reduce latency and memory usage, existing methods often degrade reasoning accuracy because selection errors accumulate over long generation horizons, or require costly retraining. We introduce LessIsMore, a training-free sparse attention mechanism for long-horizon reasoning. Our key insight is that token importance in reasoning is global and stable: critical tokens are largely shared across attention heads and remain stable over decoding steps. Guided by this structure, LessIsMore enforces cross-head unified token selection and preserves recent context via a stable recency window, yielding a globally consistent token set that can be reused across layers. Across multiple model families and challenging reasoning benchmarks, LessIsMore matches or improves accuracy while attending to substantially fewer tokens. With kernel-level optimizations, LessIsMore achieves up to $1.6\times$ end-to-end decoding speedup and up to $1.72\times$ faster sparse attention computation, with additional long-context results demonstrating the generality of our approach. Code is available at \href{https://github.com/DerrickYLJ/LessIsMore}{https://github.com/DerrickYLJ/LessIsMore}.

==> src/figs/experiments/efficiency/efficiency_e2e.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{src/figs/experiments/efficiency/e2e_efficiency.pdf}
    \caption{Efficiency-accuracy tradeoff comparison on AIME-24 using LLama-3.1-8B. Each point represents the average decoding latency across the corresponding average generation length in \Cref{tab:gen_len}. \Sys (orange squares) consistently achieves higher accuracy than TidalDecode (blue circles) while maintaining lower latency across all token budgets (1K, 2K, 4K, 6K). The closer to the top-left corner, the better the method performs. Full Attention baseline (triangle) provides the accuracy upper bound but with higher computational cost.}
    \label{fig:e2e_curve}
\end{figure}


==> src/table/rebuttal/baseline_variance.tex <==
\begin{table}[h!]
\centering
\caption{\textcolor{black}{The variance of AIME-24 accuracy on Qwen3-8B with different sample sizes over 100 passes. The sampled variance of AIME-24/25, MATH500, and GPQA stay minimal ($<$0.6) with 64, 8, and 16 samples per problem.}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{clrrr}
\toprule
Model (Task) & Task / Sample Size & 8 & 16 & 64 \\
\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Qwen-3-8B\\ (Variance)\end{tabular}}
& AIME-24 & $\pm$1.54 & $\pm$0.98 & $\pm$0.56 \\
& AIME-25 & $\pm$1.76 & $\pm$1.12 & $\pm$0.58 \\
& MATH500 & $\pm$0.14 & $\pm$0.11 & $\pm$0.05 \\
& GPQA & $\pm$0.59 & $\pm$0.43 & $\pm$0.20 \\
\bottomrule
\end{tabular}
}
\label{tab:variance_eval}
\end{table}

